End-to-End Training Approaches for Discriminative Segmental Models

Recent work on discriminative segmental models has shown that they can achieve competitive speech recognition performance, using features based on deep neural frame classifiers. However, segmental models can be more challenging to train than standard frame-based approaches. While some segmental models have been successfully trained end to end, there is a lack of understanding of their training under different settings and with different losses. We investigate a model class based on recent successful approaches, consisting of a linear model that combines segmental features based on an LSTM frame classifier. Similarly to hybrid HMM-neural network models, segmental models of this class can be trained in two stages (frame classifier training followed by linear segmental model weight training), end to end (joint training of both frame classifier and linear weights), or with end-to-end fine-tuning after two-stage training. We study segmental models trained end to end with hinge loss, log loss, latent hinge loss, and marginal log loss. We consider several losses for the case where training alignments are available as well as where they are not. We find that in general, marginal log loss provides the most consistent strong performance without requiring ground-truth alignments. We also find that training with dropout is very important in obtaining good performance with end-to-end training. Finally, the best results are typically obtained by a combination of two-stage training and fine-tuning.

==> append.tex <==
\appendix

\section{Appendix}

\begin{table}
\caption{Frame error rates for different encoder architectures.}
\begin{center}
\begin{tabular}{llll}
         & feat     & dev      & test     \\
\hline
LSTM 256x3 +dropout
         & MFCC     & 21.09    & 21.36    \\
LSTM 256x3 +dropout
         & fbank    & 20.41    & 21.26
\end{tabular}
\end{center}
\end{table}

\begin{table}
\caption{Phone error rates for segmental models
    based on log probabilities from different encoder architectures.}
\begin{center}
\begin{tabular}{llll}
         & feat     & dev      & test     \\
\hline
LSTM 256x3 +dropout
         & MFCC     & 21.9     & 22.5     \\
LSTM 256x3 +dropout
         & fbank    & 21.0     & 22.8
\end{tabular}
\end{center}
\end{table}

\begin{table}
\caption{Phone error rates for segmental models trained end to end initialized from
    the best two-stage system.}
\vspace{0.3cm}
\begin{center}
\begin{tabular}{lll}
         & dev        & test      \\
\hline
hinge    & 20.4       & 21.9      \\
log loss & 21.1-      &           \\
latent hinge
         &            &           \\
marginal log loss
         &            &
\end{tabular}
\end{center}
\end{table}


